LEMIX: Enabling Testing of Embedded Applications as Linux Applications (Extended Report)

Dynamic analysis, through rehosting, is an important capability for security assessment in embedded systems software. Existing rehosting techniques aim to provide high-fidelity execution by accurately emulating hardware and peripheral interactions. However, these techniques face challenges in adoption due to the increasing number of available peripherals and the complexities involved in designing emulation models for diverse hardware. Additionally, contrary to the prevailing belief that guides existing works, our analysis of reported bugs shows that high-fidelity execution is not required to expose most bugs in embedded software. Our key hypothesis is that security vulnerabilities are more likely to arise at higher abstraction levels. To substantiate our hypothesis, we introduce LEMIX, a framework enabling dynamic analysis of embedded applications by rehosting them as x86 Linux applications decoupled from hardware dependencies. Enabling embedded applications to run natively on Linux facilitates security analysis using available techniques and takes advantage of the powerful hardware available on the Linux platform for higher testing throughput. We develop various techniques to address the challenges involved in converting embedded applications to Linux applications. We evaluated LEMIX on 18 real-world embedded applications across four RTOSes and found 21 new bugs in 12 of the applications and all 4 of the RTOS kernels. We report that LEMIX is superior to existing state-of-the-art techniques both in terms of code coverage (~2x more coverage) and bug detection (18 more bugs).

==> figures/continuous_task.tex <==
\begin{figure}[t]
\centering
%\includegraphics[width=1.0\linewidth]{images/faultinj.pdf}
\includegraphics[scale=0.5]{images/continuous_task.pdf}
\caption{In this continuous application example of a closed-loop temperature control system, tasks 1, 2, and 3 are managed by the RTOS scheduler via timer interrupts. Task 1 reads temperature, Task 2 executes a control algorithm, and Task 3 adjusts the actuator continuously. Task 4, handles communication with an external system, is non-continuous and triggered by events or set intervals.}
\label{fig:continuous_task}
\end{figure}

==> figures/evaluation_additional_instrumentation.tex <==
\begin{figure}[t]
\centering
 \includegraphics[scale=0.5]{images/eval_additional_ins.pdf}
\caption{Placeholder line chart representing the improvements in coverage with additional instrumentation.}
\label{fig:eval_additional_ins}
\end{figure}

==> figures/evaluation_coverage_analysis.tex <==
\begin{figure}[t]
\centering
 \includegraphics[scale=0.5]{images/eval_cov_analysis.pdf}
\caption{Placeholder figure to represent coverage variations averaged across 20 different applications from 4 different RTOSes between application and function level fuzzing}
\label{fig:eval_cov_analysis}
\end{figure}

==> figures/lemix_design_phase1.tex <==
\begin{figure}[t]
\centering
%\includegraphics[width=1.0\linewidth]{images/faultinj.pdf}

% Image Link : https://drive.google.com/file/d/1-SyioSd5JLfFQVa2Uw8kJWaRaJwDIs43/view?usp=sharing
 \includegraphics[scale=0.5]{images/lemix_design_phase1.pdf}
\caption{This figure shows phase 1 of Lemix's design. The embedded application's source is recompiled to capture compile commands, cleaned of unsupported flags, and passed to the Porting Engine. Errors during x86 recompilation are analyzed, with feedback provided if not auto-fixed. The process repeats until all errors are resolved, generating bitcode files.}
\label{fig:lemix_design_phase1}
\end{figure}

==> figures/lemix_design_phase2.tex <==
\begin{figure}[t]
\centering
%\includegraphics[width=1.0\linewidth]{images/faultinj.pdf}

 % Image link : https://drive.google.com/file/d/1GLOjzsWA418XVLNabklDJPyj6RBjIhBR/view?usp=sharing
 \includegraphics[scale=0.5]{images/lemix_design_phase2.pdf}
\caption{This figure shows phase 2 of Lemix's design. In this phase, the RTOS kernel is configured for the POSIX board using the Linux Portable Layer. Necessary configurations (e.g., enabling SPI) are applied, and the RTOS kernel is compiled for a demo application, generating the corresponding bitcode files.}
\label{fig:lemix_design_phase2}
\end{figure}

==> figures/lemix_design_phase3.tex <==
\begin{figure}[t]
\centering
%\includegraphics[width=1.0\linewidth]{images/faultinj.pdf}
% Image link : https://drive.google.com/file/d/11flTJ1Hv6mcqlL1gdhHSU24YAU6-Q492/view?usp=sharing
 \includegraphics[scale=0.5]{images/lemix_design_phase3.pdf}
\caption{In the final phase of Lemix's design, the Target Application bitcode files are integrated with the compatible RTOS bitcode files coupled with the Linux Portable Layer. The outcome of this phase is the final ported application which can now be analyzed with traditional security analysis techniques.}
\label{fig:lemix_design_phase3}
\end{figure}

==> figures/mmio_old_figure.tex <==
\begin{table}[t]
\footnotesize
\renewcommand{\arraystretch}{0.9}
\setlength{\tabcolsep}{4pt}
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\toprule
\textbf{App} & \textbf{Total} & \textbf{In} & \textbf{Not in} & \textbf{SVD} & \textbf{Potential} \\
& \textbf{MMIOs} & \textbf{SVD} & \textbf{SVD} & \textbf{Detection (\%)} & \textbf{MMIOs (\%)} \\
\midrule
\rowcolor[HTML]{EFEFEF} f1 & 45 & 11 & 34 & 24.44 & 75.56 \\
f2 & 33 & 16 & 17 & 48.48 & 51.52 \\
\rowcolor[HTML]{EFEFEF} f3 & 35 & 18 & 17 & 51.43 & 48.57 \\
f4 & 15 & 11 & 4 & 73.33 & 26.67 \\ 
\rowcolor[HTML]{EFEFEF} f5 & 15 & 11 & 4 & 73.33 & 26.67 \\ 
\midrule
n1 & 8 & 4 & 4 & 50.0 & 50.0 \\
\rowcolor[HTML]{EFEFEF} n2 & 10 & 5 & 5 & 50.0 & 50.0 \\
n3 & 9 & 4 & 5 & 44.44 & 55.56 \\
\rowcolor[HTML]{EFEFEF} n4 & 9 & 4 & 5 & 44.44 & 55.56 \\
n5 & 60 & 9 & 51 & 15.0 & 85.0 \\ 
\midrule
\rowcolor[HTML]{EFEFEF} z1 & 10 & 4 & 6 & 40.0 & 60.0 \\
z2 & 10 & 5 & 5 & 50.0 & 50.0 \\ 
\rowcolor[HTML]{EFEFEF} z3 & 54 & 25 & 29 & 46.3 & 53.7 \\ 
\midrule
t1 & 16 & 6 & 10 & 37.5 & 62.5 \\
\rowcolor[HTML]{EFEFEF} t2 & 16 & 6 & 10 & 37.5 & 62.5 \\
t3 & 3 & 1 & 2 & 33.33 & 66.67 \\
\rowcolor[HTML]{EFEFEF} t4 & 16 & 6 & 10 & 37.5 & 62.5 \\ 
t5 & 16 & 6 & 10 & 37.5 & 62.5 \\
\bottomrule
\end{tabular}
\caption{MMIO detection analysis showing potential undocumented peripherals in SVD files. SVD Detection represents the percentage of MMIOs documented in SVD files, while Potential MMIOs shows the percentage of detected MMIOs that may also represent legitimate peripherals not documented in SVD files.}
\label{tab:mmio_table}
\end{table}

==> figures/overview.tex <==
\begin{figure}[t]
\centering
%\includegraphics[width=1.0\linewidth]{images/faultinj.pdf}
\includegraphics[scale=0.7]{images/Overview.pdf}
\caption{
  Overview of our Approach and Associated Challenges.
  The rehosted system consists of the application components, the~\ac{RTOS}, and the other SDK components.
  The main challenges are (1) building this rehosted application, (2) preserving the execution semantics, and (3) handling peripherals.
  % \JD{Write (1), (2), (3) to map to the figure.}
  % \JD{The figure says ``Challenge 2'' and ``Challenge 3'' but not ``Challenge 1''.}
  % \JD{It is a little hard to see the ``Challenge X'' words in the figure. Can you increase font size and italicize?}
  % \JD{Some words are too small, like ``Invoke handler'' and ``Peripheral access''}
  }
\label{fig:overview}
\end{figure}
%\vspace{-0.10cm}

% source for this figure: https://drive.google.com/file/d/1NgKWL7CUzpREx2VlOMi7O5tbp__C_pwS/view?usp=sharing

==> figures/rehosting_fidelity.tex <==
\begin{figure}[t]
\centering
%\includegraphics[width=1.0\linewidth]{images/faultinj.pdf}

% Image Link : https://drive.google.com/file/d/1ZX3gOklCpDBXDpz-BxdgZ7sfmhGeX_cc/view?usp=sharing
 %\includegraphics[scale=0.5]{images/rehosting_fidelity.pdf}
 \includegraphics[scale=1.0]{images/rehostingfidelity-new.pdf}
 \vspace{-0.5cm}
\caption{Comparison of existing techniques with \systemname{} and Bug Manifestation Fidelity.}
\label{fig:fidelity}
\end{figure}

==> figures/threat_model.tex <==
\begin{figure}[t]
\centering
% Image link  : https://drive.google.com/file/d/11Ws7YYvFUQL2ocFZrKJpzJ7oQWjbfNhL/view?usp=sharing 
\includegraphics[scale=0.3]{images/threat_model.drawio (3).pdf}
\vspace{-0.5cm}
\caption{
Lemix's threat model assumes malicious inputs from both Peripheral MMIO accesses and Inputs when Interrupt Service Routines are triggered in embedded applications.
\iffalse
\JD{The font size in this figure is far smaller than the font size in the manuscript. That is a formatting violation.}
\JD{If this is the main overview figure, then the approximation aspect should be indicated.}
\fi
}
\label{fig:threat_model}
\end{figure}

==> listings/bug.tex <==
\begin{listing}
\inputminted[linenos, mathescape, escapeinside=@@, fontsize=\scriptsize{}]{cpp}{code/bug.c}
\caption{Division By Zero Error: Value \textit{pllm} is read from a peripheral register and used as divisor without any check (\textcolor{red}{\faBug}).}
\label{lst:bug}
\end{listing}
\vspace{-0.08cm}

==> listings/identified_bugs_2.tex <==
\begin{listing}
\begin{minted}[xleftmargin=0.25cm, numbersep=1pt, escapeinside=||, fontsize=\scriptsize, breaklines, linenos]{cpp}
    uint32_t tud_msc_read10_cb(uint32_t lba, 
        uint32_t offset, void* buffer, uint32_t bufsize)
    {
      // out of ramdisk
      if ( lba >= DISK_BLOCK_NUM ) return -1;
      // Missing bounds check
      uint8_t const* addr = msc_disk[lba] + offset; |\textcolor{orange}{\faExclamationTriangle}|
      // Potential buffer overflow due to unchecked 
      // offset+bufsize
      memcpy(buffer, addr, bufsize); |\textcolor{red}{\faBug}|
      return bufsize;
    }
\end{minted}
\caption{Missing bounds check for addition of offset and bufsize \textcolor{orange}{\faExclamationTriangle} in tud\_msc\_read10\_cb can lead to buffer overflow \textcolor{red}{\faBug} during memcpy operation.}
\label{lst:identified_defects_2}
\end{listing}

==> listings/ifcond.tex <==
\begin{listing}
\inputminted[fontsize=\scriptsize{}]{cpp}{code/isr.c}
\caption{The handler consists of highly constrained checks on the register values before trying to read from the USART (peripheral).}
\label{lst:constraint}
\end{listing}

==> listings/motivation_bug.tex <==
\begin{listing}
    \begin{minted}[xleftmargin=0.25cm, numbersep=1pt, escapeinside=||, fontsize=\scriptsize, breaklines, linenos]{cpp}
    
    size_t board_get_unique_id(
        uint8_t id[], 
        size_t max_len
    ) 
    {
      (void) max_len;
    
      // MMIO Access, controlled by attacker
      uintptr_t did_addr = 
                NRF_FICR->DEVICEID; |\textcolor{orange}{\faUserSecret}|
    
      const uint8_t* device_id = 
                (const uint8_t*) did_addr; |\textcolor{orange}{\faUserSecret}|
      for(uint8_t i=0; i<8; i++) {
        // Arbitrary data write to id memory
        id[i] = device_id[i]; |\textcolor{red}{\faBug}|
      }
      return 8;
    }
\end{minted}
\caption{The device ID is read from \textit{NRF\_FICR} and used without validation, risking NULL pointer dereferencing or arbitrary writes.}
\label{lst:motivation_bug}
\end{listing}

==> sections/acknowledgements.tex <==
\section*{Acknowledgment}
We gratefully acknowledge support from Rolls Royce.

==> sections/challenges.tex <==
\input{tables/fulldatasettable}

==> sections/feasibility.tex <==
\section{Feasibility Study}
\label{sec:feasibility}

\input{listings/bug}

We assessed the feasibility of our approach by applying it to~\numapp{} real-world applications based on FreeRTOS~\cite{FreeRTOS}.

\textit{\textbf{InfiniTime}}: A smart watch application~\cite{Infinitime} based on nrf52 microcontroller. It uses many libraries --- LVGL for UI, NimBLE for its BlueTooth Stack, and JetBrains for fonts.

\textit{\textbf{TinyUSB demo}}: A demo application of TinyUSB~\cite{TinyUSB}, a popular cross-platform USB Host/Device stack for embedded systems that runs on feather\_nrf52840\_express board.

\textit{\textbf{SmartSpeaker}}: A smart speaker application~\cite{SmartSpeaker} using stm32f407vet6, wm8978, and esp8266 for master control, audio DA/ADC, and network communications, respectively.

\vspace{0.05cm}
We converted each of the above applications into Linux applications using our approach (\sect{sec:overview}).
Specifically, we built the applications using the Linux port of FreeRTOS, by using compiler flags with that of~\targetarch{}~\clang{}.
We then manually identified all~\ac{MMIO} accesses and replaced them with reads from standard input.
Finally, we created our interrupt dispatcher task that invokes one of the registered interrupt handlers based on a value read from standard input.

\vspace{0.05cm}
\noindent\textbf{Preliminary Evaluation:}
We compiled each of these applications using ASAN~\cite{serebryany2012addresssanitizer} and executed them on Ubuntu 20.04 machine.
% These applications executed fine without any crashes, and we verified through a debugger that the applications were indeed executing as expected. %TOCHECK
The application tasks executed as expected without undefined crashes. % which we validated on a debugging environment.
Accesses to peripheral regions did not fault.
Execution proceeded as input was provided via standard input.


\emph{Testing:} To check the robustness and bug-exposing ability of these rehosted applications, we tested them using~\afl~\cite{afltech} for~\fuzztime{} hours. 
We found two previously unknown floating-point exceptions in the STM32 driver code~\cite{Stm32Library} --- in the Clock module and in the SPI driver.

As seen in ~\lst{lst:bug}, %TOCHECK%
the value \texttt{pllm} is read from a member of \texttt{RCC} peripheral register (line 5).
 On line 12, it is used as a divisor without any check for zero.
STM32 has fixed the bug \cite{Stm32LibraryBug} in their latest release.

\iffalse
\subsection{Building with Linux Port}
%--Say what steps you followed for 3 applications to convert into Linux applications--Build related things--

The process of building the applications involved manually inspecting the build arguments and creating a custom Makefile by including all the relevant sources and compilation flags. The FreeRTOS kernel and required headers were then added to the Makefile along with any necessary changes for the specific SDK like defining the MCU used. The main change with respect to the sources is that the~\ac{MCU}-specific portable layer is changed to the Linux counterpart along with relevant memory management files. We chose clang as our compiler since it provides many instrumentation capabilities with its backend LLVM part. Therefore compilation issues including those specific to clang like static asserts, incorrect pointer casts, and unknown members in namespaces were addressed. Additionally, for the compilation to occur successfully, we manually commented out inline assembly. 

\subsection{Maintaining Event-driven Execution}
%--Say how we handle interrupts in these applications--
We trigger the interrupts in a randomized fashion. 
A new task called the Interrupt handler task is created alongside the other application tasks which periodically triggers one of the interrupt service routines with high scheduling priority. 
This ensures that the interrupt task is provisioned first by the \ac{RTOS} thus mimicking a context switch. 

\subsection{Peripheral Handling}
%--How did we identify peripheral access? Manually using grep.
We identified all the peripheral registers from the board configuration file that is included as part of the SDK. 
For each peripheral defined in the configuration, we manually found all its access instances in the code base using \textit{grep}.
%--Say that you replaced each MMIO read with scanf and commented out MMIO write--
If the access was a read, we included a stub code so that the read happens through standard input. 
For a write, however, we ignore the access by commenting it out.
\fi

==> sections/lemixdesign.tex <==
\section{Implementation}
% \ritvik{Ready for review}

% \machiry{Here goes the details of our 1st phase.}

\subsection{Converting to a Linux Application}
\label{subsec:porting}
% What are the steps in conversion?

% \machiry{Fill in the details.}

\subsubsection{Capture Compilation Commands:} 

To mimic the build process, \systemname{} begins by building the application using its original build instructions. During this step, we use Bear~\cite{bear} to capture the compilation commands invoked by the original build system for each source file. By capturing these commands, we also record any compile-time macros passed during compilation, eliminating the need to manually include them in our build, as they are already part of the captured \textit{compile\_commands.json}. Since embedded build systems often rely on custom tools and wrappers (e.g. \textit{ fbt} for Flipperzero), Bear helps standardize the porting process thereby enabling rehosting build procedures to use the regular Unix Makefile. We replace the native architecture compiler with the x86-32 clang and use wllvm~\cite{wllvmtool} as a clang wrapper to generate LLVM bitcode files for instrumentation analysis. After cleaning the compilation commands (e.g., removing clang-incompatible flags), we recompile to produce x86-equivalent object files for each source.

\input{tables/gcc_clang_differences}

\input{listings/inlineASM}

\input{listings/hexASM}

\subsubsection{Human-In-Loop Approach to Resolve Compilation Errors:}
~\systemname{} monitors the compilation process and fixes any errors which are caused by known issues. Some of the common issues which framework resolves in a semi-automated way are - 

\subsubsection*{(1) GCC vs Clang Incompatibilities:}
\label{subsec:compiler_diffs}

A significant portion of open-source embedded software relies on GCC-based toolchains~\cite{von2011definitive}, making the transition from a GCC build environment to Clang challenging. Table~\ref{tab:gcc_clang_diffs} highlights several incompatibilities between GCC and Clang~\systemname{} that we identified during the process of porting. Although clang's official documentation does highlight some of the incompatibilities of Clang against GCC~\cite{LanguageCompatibility}, we believe we are the first to highlight these issues in the embedded domain, which have not yet received sufficient attention among embedded developers. Addressing these incompatibilities can help facilitate effective cross-compiler compatibility. Issues like Variable-Sized Object initialization are still not supported even in the latest version of LLVM at the time of writing (LLVM 18)~\cite{dgookin_2023}. The table also highlights challenges such as absence of certain symbols like \textit{\_\_assert\_func} which are internal to Arm GCC's intrinsic header files. For these symbols, we capture their corresponding definitions from the original source's preprocessor output. We create a global header file which is then included in the subsequent compilation. Most of the compiler error fixing is automated via pattern matching and patching source code with accurate fixes, examples of which are provided in Table~\ref{tab:gcc_clang_diffs}. However, for other issues which we could not automate,~\systemname{} provides hints to developers to assist in fixing them.

\subsubsection*{(2) Handling Inline Assembly:}
% \ritvik{Add challenges wrt how hard it is to identify inline asm on source level - say how clang AST parser fails to grab ASM from inside macros and source level parsing to extract such ASM is tedious task.}
Our observations indicate that most \ritvik{Quantify how much} inline assembly in embedded applications is used for board-specific startup and initialization. This step is generally not necessary for the application to function as intended on the Linux platform. \systemname{} identifies all such assembly snippets throughout the application's code base and nops them during compilation. Identifying inline assembly at the source level poses challenges, especially when it is embedded within macros. Tools like Clang’s AST parser often fail to extract inline assembly from such constructs, making source-level parsing complex and labor-intensive. Due to the complexity of inline assembly representation, \systemname{} may occasionally miss inline assembly in macro definitions. In such cases, developer assistance, guided by \systemname{}'s hints, may be needed to address the issue. The framework detects inline assembly based on pattern matching and other similar techniques, but there are other different ways in which application developers choose to depict inline assembly. Listing~\ref{lst:hexASM} shows a snippet from a function which uses hexadecimal code to represent inline assembly.~\systemname{} is capable of identifying this type of assembly based on how this hex code is used (as a function pointer in this example). We also observed that some applications use inline assembly functions to optimize reading values from architecture-specific registers, as shown in Listing~\ref{lst:inlineASM}. These values are often used in various program-specific initialization checks. Currently, we over-approximate these reads by returning 0 or 1 based on random numbers. While this approach can potentially lead to false positive crashes or unintended application behavior, we hypothesize that over multiple runs, this approximation will allow the application to overcome initialization routines where it might otherwise result in unexpected behaviour. 

\subsubsection*{(3) Identify ISRs and Integrate ISR Task:}
To ensure an embedded application runs correctly on a Linux platform, we insert an Interrupt Triggering Task. It operates alongside other tasks, periodically issuing interrupts to mimic real-time scenarios. If the application adheres to our requirements (See Section~\ref{subsec:app_requirements}), we identify all triggerable interrupt routines through the Interrupt Vector Table, typically located in board-specific startup files. \systemname{} filters interrupts based on whether calling the ISR directly from within the application's task would leave the application in an inconsistent state. This is determined by ensuring that the global structures responsible for handling the interrupt are properly initialized ~\ritvik{Include a listing showing uninitialized ISRs}. The task creation and scheduler checking APIs must be manually identified when porting applications to a new RTOS.

\subsubsection{Posix Swap}
After porting the application source files to x86, ensuring utilization of the Linux Portable Layer (LPL) in the underlying RTOS is crucial. This translates application-level semantics effectively into the POSIX environment. \systemname{} compiles a sample application separately for the POSIX board to utilize LPL. This process provides RTOS kernel files configured for the POSIX platform. We term this procedure as POSIX swap.

However, the original build instructions of the application may include board-specific configurations enabling certain HAL-specific APIs necessary for its function. Sometimes, peripheral models implemented in the original RTOS may not be available in the corresponding LPL, as discussed in Section~\ref{subsec:portability_layers}.

Addressing these challenges, \systemname{} selectively incorporates configurations from the application that do not disrupt the POSIX build. Each RTOS configuration is iteratively toggled in the POSIX build, saving configurations that compile successfully. Once the POSIX build incorporates necessary application configurations without issues, \systemname{} replaces the application's RTOS kernel files with those from the successful POSIX build.

\subsubsection{Resolve Linker Level Errors}

After the POSIX Swap, the final phase in porting an application is linking all object files. Replacing RTOS kernel object files with POSIX Kernel object files introduces two challenges~\ritvik{This approach can be explained algorithmically}:
\begin{itemize}
    \item \textbf{Undefined reference errors:} Occur when symbols referenced in the board-specific RTOS kernel files are absent in the POSIX Kernel files post POSIX swap.
    \item \textbf{Multiple reference errors:} Arise when symbols are duplicated across the swapped POSIX kernel files and the remaining application RTOS files.
\end{itemize}

\subsubsection*{(1) Resolving Undefined References}

To resolve undefined references, the framework looks for the corresponding application kernel object files which have this symbol defined. Bringing in this application kernel object file into linking can cause other multiple reference errors due to the symbols being defined in both application and the POSIX RTOS file. Some symbols like \emph{\_\_compiler\_barrier} are internal to the target architecture compiler for which we create dummy function signatures and empty bodies~\ritvik{Our Goal here is to maintain decent fidelity to enable security analysis on apps, so this is ok to do}. 

\subsubsection*{(2) Resolving Multiple References}
To resolve multiple references,~\systemname{} follows 2 phases. 

\begin{itemize}
    \item \textbf{Creating Library Archives :} By following the original build procedure of an application step by step, we observed that library archives are created by grouping certain object files together and are included during linking. This helps in linking object files of different modules where some object files in a module may have a symbol weakly defined whereas strongly defined in others. Archiving an object file with weakly defined symbol prevents occurrence of multiple reference errors ~\ritvik{Give an example of how RTOS apps use archiving.} .~\systemname{} identifies all the library archives that were created in the original build, thereby also capturing the information about which files have to be archived. This resolves large majority of multiple reference errors.

    \item \textbf{Modifying Symbol in One of the Objects:} The remaining multiple references cannot be resolved by archiving, hence the symbol name has to be modified in one of the object files. If the multiple reference is between an Application's object file~\ritvik{By App, we mean App + App kernel + App HAL} and POSIX kernel object file, we pick the Application object file for symbol modification; this is to ensure that we retain any calls that the application API makes into the POSIX layer of the RTOS. For other cases, we modify either of the object files to resolve the error.
\end{itemize}


\subsubsection{Handling RTOS Standard Library Calls}

Amidst our efforts in rehosting the application, we identified that, for an application to function as intended on a POSIX board, we must mimic the behavior introduced by the linker in symbol renaming when compiling a sample application for POSIX board. Mature RTOSes such as Nuttx and Zephyr employ sophisticated symbol management and linking strategies to handle the dual-context execution between the RTOS environment and the host system. This architecture creates a clear separation between the calls of RTOS standard library functions from the host through a specialized linking process. To mimic this behavior in our ported applications, we read the Global Offset Table (GOT) entries of the sample application to identify functions that should be directed to the host standard library. This allows us to determine which calls should be redirected to the application and which should be directed to the RTOS standard library.

\subsubsection{Handling Symbol Aliasing}
During testing of the ported application, we discovered that several null pointer dereference crashes were caused by attempts to call aliased symbols. In the original application's build procedure, the linker creates aliases for various symbols to maintain interoperability across different boards as guided by linker scripts. For instance, the symbol \textit{\_\_init\_clock} might be resolved to aliases like \textit{\_\_stm32\_clock\_init} or \textit{\_\_nrf52\_clock\_init}, depending on the target board. Additionally, multiple aliases can be created for the same symbol, further complicating our rehosting efforts. To address this, \systemname{} extracts aliasing information from the original ELF compiled for the board by loading the ELF in GDB and verifying which symbol each alias points to. With this information, our instrumentation passes ensure that all such aliases are correctly redirected to their original references at link time.




% \subsubsection*{(f) Handling Library Calls}

% \ritvik{Need to fill this now that it's done!}

% To preserve application fidelity on top of instrumentation, ~\systemname{} ensures that all calls to standard library are redirected to the application standard library (if one exists or is provided by the RTOS kernel). 

% \begin{itemize}
%     \item Capture Compilation Commands
%     \item Retarget for x86 ISA and handle inline assembly.
%     \item Resolve GCC vs Clang Issues.
%     \item Identify ISRs and Insert ISR Task.
%     \item Identify portable layer and replace with LPL.
%     \item Resolve Linker Level Errors.
%     \item Add stub methods for missing functions.
% \end{itemize}
\subsection{Handling Peripheral Interactions}

To handle peripheral interactions, \systemname{} performs the following 2 steps - 

\subsubsection{Constant Address Analysis}
Most MMIO address references in the ported application are constants. Our analysis identifies such constants in operands of load and store instructions, as well as constant arguments in function calls. We focus on addresses greater than 4 bytes and below the 32-bit userspace stack range to detect most MMIOs. Although some non-MMIO constants may also be flagged as MMIOs, providing input from stdin to these non-MMIO loads does not affect program behavior, as these constants are simply numbers and are not mapped to the ELF userspace in any way. Once we identify an MMIO address, we mask its value to the nearest page boundary. We then treat all MMIO accesses within a range of ±2 KB from that boundary as MMIOs. This approach helps group related MMIO accesses and ensures that accesses within the same memory-mapped region are consistently recognized.
% \begin{itemize}
%     \item Find constant addresses.
%     \item Coalescing adjacent Pages.
% \end{itemize}
\subsubsection{Memory Access Instrumentation}
We instrument all memory loads and stores so that the loads read from the standard input.

\subsection{Assisting Dynamic Analysis}

\PA{I think there should be a subsubsection here as this paragraph is about one effort to assist dynamic analysis. The subsection paragraph should provide an overview of the different efforts the subsection talks about}

As demonstrated by Liyanage et al.~\cite{reachableCoverage}, focusing on reachable coverage elements is key to enhancing fuzzing effectiveness by ensuring that only reachable code paths are tested. Building on this insight, we introduce a customized coverage metric for application-level fuzzing that focuses on all reachable functions from \textit{main} and \acp{ISR} injected by \systemname{} during the porting process. AFL++'s coverage, which reports the coverage of the entire program—including modules from the application’s kernel, the HAL, and the POSIX kernel—does not align well with our scenario. This broader coverage can be inaccurate, as it may include functions that are not reachable from the application's perspective. Our linking procedure brings in additional application kernel files to resolve undefined references, which may contain functions unused by the ported application.

\subsubsection{Reachability Analysis For Precise Coverage Measurement}

Our analysis traverses call graphs on the basic block level via LLVM IR and identifies all the functions reachable from \textit{main} and the ISRs that are injected by \systemname{}. However, when applications do not comply with our system requirements (see Section \ref{sec:threat_model}) and no ISRs are injected, we only get the reachable functions from main.

\subsubsection{Weakening data-independent conditions}

\input{listings/branch_instrument}

Our analysis found that certain conditions depend on MMIO values, creating constraints that AFL struggles to solve within a reasonable timeframe. Listing \ref{lst:blocker} illustrates one such constraint, which halts fuzzing thereby hindering our efforts in effective dynamic analysis of the application. While AFL++ could eventually resolve these constraints given enough time, they frequently appear early in board initialization routines, causing the application to remain stuck without progress. To address this, inspired by prior work \cite{choi2019grey}, we simplify MMIO-dependent constraints. Our instrumentation identifies such branches and modifies them to be controlled by \textit{stdin \% 2}, toggling the condition with a 50\% probability to give AFL a fair chance to explore both the if and else paths.

\section{Application Level Fuzzing}

We compile the instrumented bitcode with Sanitizers and use our modified AFL++ to fuzz the ported applications under persistent mode. Every MMIO access we have modeled will receive mutated inputs from AFL. Without any instrumentation, in configuration \textit{C0}, we observed that applications even failed to run RTOS related initialization tasks and result in no coverage. \textit{C1} configuration is coverage without any branch instrumentation or cross-function MMIO tracking, and \textit{}{C2} is coverage with data independent branches instrumented and cross-function MMIO tracking. Weakening of data independent conditions helps AFL cover more paths as can be seen in the coverage differences between both configurations of \systemname{} in Table~\ref{tab:tool_eval}. Our original coverage metric is source line coverage, which had to be normalized to basic block coverage to compare against existing works. \textit{C3} configuration is~\systemname{}'s application level coverage added to the unique number of basic blocks identified via function level fuzzing in functions that were not covered by application level fuzzing in \textit{C1}.

\section{Function Level Fuzzing}
Given a function, we will automatically create fuzzing harness.

\subsection{Type Inference and Co-Relation Analysis}

Type inference involves automatically identifying the types of inputs, outputs, and internal variables in a function.
This is crucial to ensure that the fuzzing harness understands the data structure and boundaries for each function. The fuzzing engine analyzes the function’s signature, its control flow, and the expected data types for each parameter.
Additionally, co-relation analysis is employed to understand how different variables or parameters within the function interact with each other.
This analysis allows the creation of relationships between the input variables and their potential effects on the function's behavior, ensuring that the generated test cases are meaningful and explore different paths within the function.

\subsection{Type Generation}

After type inference, type generation focuses on producing valid input values for the identified types.
This process involves mutating the inputs to cover a wide range of test cases, from edge cases to typical scenarios, while respecting the type constraints identified in the previous step.
For example, if a function accepts an integer, the type generation process will create a range of integers, including negative numbers, large values, and boundary cases.
If the function accepts a pointer or reference type, the type generation will include valid and invalid memory addresses.
The goal is to generate a comprehensive set of inputs that stress-test the function's handling of various types, ensuring that vulnerabilities or undefined behaviors are uncovered.

\subsection{Function Fuzzing}

Each target function is isolated into a standalone executable by accurately setting up its runtime environment, including arguments, global variables, and mocked dependencies, ensuring it is self-contained and behaves as expected.
A non-crashing seed input, identified automatically, is used as the input for AFL++, which further generates mutated inputs to explore various execution paths. Integrated sanitizers then detect and report any crashes or undefined behavior, enabling comprehensive vulnerability triaging.



==> sections/oldcontent.tex <==
\section{OLD CONTENT}

%Explain the overview of our approach using the overview figure.
% TODO: DESCRIBE THE PROBLEM BEFORE THE SOLUTION
%Rehosting enables the embedded application to execute without the actual hardware by emulation which requires an underlying engine to support the \ac{MCU} architecture. However, with different \ac{MCU} families being introduced, providing additional support for these in the emulation engine becomes very difficult.
%We achieve rehosting of Type-2 embedded systems into a Linux application using the portable layer of ~\ac{RTOS} that does away with the need for an emulator. As seen in ~\fig{fig:overview}, application components, third-party SDK, and libraries including the ~\ac{OS} become part of the executable in our rehosted system. 
% Explain the two challenges and how to solve each of them:
%The challenges that come with rehosting this way are building the Linux application, preserving the execution 
%semantics, and handling the peripheral interactions. 
This section summarizes our approach to rehosting an embedded application as a Linux application.
\fig{fig:overview} shows an embedded application rehosted as a Linux application using our approach to handling the three challenges.

\input{figures/overview}

\subsection{Retargeting for a general-purpose ISA (\targetarch{})}
% \davis{This paragraph says ``we made a mapping between compiler flags''. It is very verbose for such a simple outcome. Perhaps we can better the space to SHOW the compiler flag mapping or some examples?}
As explained in~\sect{sec:introduction}, to compile an application for \targetarch{}, we need to handle: (a) Toolchain differences between~\ac{MCU} specific compiler and the~\targetarch{} compiler. (b) Inline assembly.
Most~\ac{MCU}s use a RISC-based~\ac{ISA} with custom toolchains suitable for the architecture of the processing unit.
These support architecture-specific options (\eg~\code{-mthumb-interwork}) and custom options (\eg~\code{-grecord-gcc-switches}), often unavailable in commodity compilers (\eg~\clang).
Consequently, naively replacing the compiler with a commodity compiler fails.
% But, just ignoring them will not work as they might be needed to achieve the desired compilation.
% Instead, we need to use the corresponding options in the~\targetarch{} compiler.
% We handle this by maintaining a mapping of the options in~\ac{MCU} and~\targetarch{} compilers and leveraging existing tools~\cite{wllvmtool}.
Using existing build interceptor tools~\cite{wllvmtool}, we replace the embedded toolchain and the dependent flags relevant to compilation and linking, with Linux equivalents in the Clang toolchain.

The presence of inline assembly code pertaining to the~\ac{MCU} architecture is a related challenge. 
We noticed that inline assembly is mostly used to access~\ac{MCU} specific registers and modify features of the~\ac{MCU}.
% These features are usually not present in~\targetarch{}.
% \davis{can we spell this ``NOPing'' or similar?}
As our main focus is on vulnerability detection, our intuition is that NOP'ing out inline assembly components would not overly hinder the overall analysis.
We therefore handle inline assembly by commenting it out from the source files.

\iffalse
\subsection{Building the Rehosted Application}
Embedded systems code is highly coupled to the hardware and cannot be directly compiled for the x86 architecture. The presence of inline assembly and the differing toolchain specifications attribute to this challenge. We observe that these assembly snippets are sparse when compared to the entire codebase, and often related to the manipulation of essential peripherals required for high-fidelity execution. Since our main focus is on vulnerability detection, nopping out inline assembly components we believe would not hinder the overall testing to a large extent. Further, to achieve the porting of the application, specific toolchain requirements like unsupported build flags are changed.
\fi

\subsection{Preserving Execution Semantics}
The second challenge is to ensure that the application components (\eg tasks) in a rehosted Linux application have the same execution semantics as in the target embedded system.

\vspace{0.03cm}
\noindent\textbf{Task-based Execution:}
% \davis{almost all? do you have data on this? that's a huge claim. ``X of the top Y'' perhaps?}- Added many RTOSes instead adding X/Y, since we have not done that analysis
We noticed that many popular~\ac{RTOS}es have a Linux port~\cite{osrtoses,OSIotLowEnd,OSLowEndIOT}, which implements the portable layer (\fig{fig:background}) using Linux-based user space libraries,~\eg providing task interface through~\code{pthreads} library APIs.
Consequently, we can have the~\ac{RTOS} compiled for Linux, where all its functions (\eg task, message queues) are implemented through Linux user space libraries.
We use these ports by compiling the embedded application using the Linux portable layer instead of the~\ac{MCU} alternative.
The resulting executable will run as a Linux application --- using existing library APIs (\eg~\code{pthread}) to achieve nearly the same execution semantics as in the original embedded system.
% 1. Preserving execution semantics: Explain the challenge (refer to intro).
% How do we handle this:

\iffalse
The rehosted application should semantically be similar to the embedded application, which means that the properties of task-based and event-driven execution must be preserved. 

\textbf{Task-based Execution:}
The rehosted system should be task-based that the \ac{RTOS} handles. 
The Linux port of the ~\ac{RTOS} inherently preserves the task-based semantics, by enabling the tasks to execute as \textit{pthreads}. 
Therefore, the ~\ac{MCU} specific portable layer is swapped with the Linux alternative along with changing relevant configurations in the ~\ac{RTOS}.
\fi
\input{listings/ifcond}

\vspace{0.03cm}
\noindent\textbf{Event-driven Execution:}
Interrupts enable event-driven execution by invoking handler functions (\lst{lst:isr}) when triggered.
These handlers are recorded in the interrupt vector table which is usually present in a~\ac{MCU} vendor-provided assembly file (\emph{eg., startup.a}).
This cannot be executed on the x86 machine.
% \JD{Next sentence is poorly phrased}
The application can register custom interrupts by adding the handler addresses to the interrupt vector table.
We recognize such interrupt-registering functions in the application and gather all the handlers.
We then create a special dispatcher task (\fig{fig:overview}) which will be invoked periodically by the RTOS scheduler. The interrupt handlers will be executed as function calls by this task as shown below:
\begin{minted}[fontsize=\scriptsize{}]{cpp}
    handlers <- array of registered handlers.
    n <- number of handlers.

    a = read_input();
    idx = a % n;
    handlers[idx](); // invoke a handler.
\end{minted}



\iffalse
Interrupts enable event-driven execution and are handled by registering routines that often contain critical application code.
Also, they are important for communication with external entities.
%--SHOW CODE EXAMPLE--.
For example, Listing~\ref{lst:isr} shows an interrupt handler that holds the essential code to transmit or receive over \texttt{UASRT1} interface with external sources. 
%--GIVE AN EXAMPLE--
The Linux port does not inherently support event-driven execution and therefore, we handle interrupts by means of a custom-created task. Specifically, we hook into the interrupt registering routine to record the addresses of the interrupt handlers.
% --SHOW CODE EXAMPLE--
% We also register a handler for the timer signal, which will be invoked periodically by Linux kernel.
This task is provided with the highest scheduling priority and acts as the main interrupt dispatcher by invoking the routines based on a value read from standard input.
\fi

\subsection{Handling Peripheral Interactions}
\label{subsec:periaccess}
Peripherals are accessed through special memory regions, called~\ac{MMIO} regions, which need to be identified and handled.

\vspace{0.04cm}
\noindent\textbf{Identifying~\ac{MMIO} regions:}
First, we need a way to distinguish~\ac{MMIO} access from normal memory access.
We observed that~\ac{MMIO} address ranges are usually hardcoded in specific source files (\eg{\emph{stm32f4xx.h}}~\cite{Stm32Library}).
Therefore, we consider these addresses, usually within a specific range that is indicated in the~\ac{MCU} datasheet as~\ac{MMIO} regions.
% \davis{hardcoded: any hardcoding, eg 0xdeadbeef, or in specific range?}

\noindent\textbf{Peripheral Access Handling:}
We analyze source files of a given application to identify accesses to~\ac{MMIO} regions.
Our threat model supposes that peripherals may be producing malicious input.
We, therefore, modify these accesses to use standard input, so that a dynamic analysis can observe the effect of different input values. 
Specifically, as we show below, all reads from these regions will be replaced with reads from standard input (\faChevronCircleLeft), and all writes will be ignored --- this is in line with our threat model (\sect{sec:background}).
\begin{minted}[mathescape, escapeinside=||, fontsize=\scriptsize{}]{cpp}
  // ...
  // Reading values from hardware registers
  // pllm = RCC->PLLCFGR & RCC_PLLCFGR_PLLM;
  pllm = |\faChevronCircleLeft|read_standard_input() & RCC_PLLCFGR_PLLM;
\end{minted}
%In principle, we are modeling peripheral accesses as reads from random memory.
% However, this may not work for essential peripherals as they need to be handled precisely to maintain the execution semantics.
The Linux port handles the execution semantics without depending on essential peripherals. Hence feeding random data to these doesn't affect the execution semantics of the rehosted application.
% \davis{I do not understand the previous two sentences. The linux port works so long as you MODEL the essential peripherals, right?}
Feeding data from standard input to non-essential peripheral accesses, such as GPIO and SPI, models the embedded application's external world interactions through standard input of the corresponding rehosted application.
\iffalse
% 2. Handling peripherals: 
% Briefly explain the challenge (Refer to the intro)
Embedded systems possess special address regions that are mapped to peripherals. Identification and handling of peripheral accesses is a major challenge. 
%Identifying peripheral accesses?

\textbf{Peripheral Identification:}
Peripheral address regions are identified using the hardware-dependent configuration file of the ~\ac{MCU}. The occurrences of these peripheral variables can therefore be looked up with this information.
% This pattern can be used to identify all peripheral accesses. %TOCHECK
% \input{listings/ifcond}
%How do we handle peripheral access?

\textbf{Peripheral Access Handling:}
Once identified, peripherals need to be handled as accesses to these addresses would be illegitimate on the rehosted system. 
We use standard input to feed data for reads instead of loading from the peripheral addresses and ignore the writes.
The Linux port handles the execution semantics without depending on essential peripherals and hence feeding random data to these would be justifiable.
Although not necessarily needed for execution, the handling of non-essential peripherals such as GPIO, SPI, etc, that aid interaction with the external world is required to enable the application to behave in certain ways.
Here, feeding random data may lead to poor dynamic coverage as the application might expect to have specific values from the peripheral.
%--GIVE AN EXAMPLE OF IF CONDITION--.
\fi
% \input{listings/ifcond}

% \begin{minted}[mathescape, escapeinside=||, fontsize=\footnotesize{}, linenos]{c}
% \end{minted}

\vspace{0.04cm}
\noindent\textbf{Handling Peripheral Access Checks:}
Peripherals use control registers to communicate the availability of data.
Applications check for specific values in control registers before trying to read data (\lst{lst:isr}).
We noticed that most of these conditions are non-data-dependent, meaning that the code within the conditional expression does not use the value in the condition.
We handle this by making such non-data-dependent MMIO access-based conditions always true.
This approach follows the previous work T-fuzz~\cite{peng2018t}, which showed that ignoring non-data-dependent conditions improves code coverage.

\iffalse
\textbf{Handling Highly Constrained Checks:}
As shown in Listing~\ref{lst:isr}, %TOCHECK
the status bits of \texttt{USART1} peripheral register is checked to determine if there is data ready to be received. 
If so, the data is placed on the \ac{RTOS} queue, which other tasks can utilize thereby improving code coverage. 
Our analysis revealed that most of these conditions in place are non-data-dependent meaning that the code within the conditional expression does not use the value in the condition.
Therefore we make the condition true so that the execution always continues.
This approach is similar to the previous work T-fuzz~\cite{peng2018t}, which demonstrated the effectiveness of ignoring such non-data dependent conditions for improving code coverage.
\fi



%\subsection{A Novel Rehosting Approach}
%JS: Placement: Page 2, 3
%Brief about RTOS and its portable layer - explain how we can change the portable layer and test it using existing well-established techniques

%Feasibility of this approach is that a major part of the application code might not be directly impacted by hardware - which is why precise emulation can be an overhaul - 

%Explain potential impact - its applicability to a whole host of systems - knowledge on hw specifics not necessarily required

==> sections/oldimplementation.tex <==
\section{Implementation}
% \ritvik{Ready for review}

% \machiry{Here goes the details of our 1st phase.}

\subsection{Converting to a Linux Application}
\label{subsec:porting}
% What are the steps in conversion?

% \machiry{Fill in the details.}

\subsubsection{Capture Compilation Commands:} 

To mimic the build process, \systemname{} begins by building the application using its original build instructions. During this step, we use Bear~\cite{bear} to capture the compilation commands invoked by the original build system for each source file. By capturing these commands, we also record any compile-time macros passed during compilation, eliminating the need to manually include them in our build, as they are already part of the captured \textit{compile\_commands.json}. Since embedded build systems often rely on custom tools and wrappers (e.g. \textit{ fbt} for Flipperzero), Bear helps standardize the porting process thereby enabling rehosting build procedures to use the regular Unix Makefile. We replace the native architecture compiler with the x86-32 clang and use wllvm~\cite{wllvmtool} as a clang wrapper to generate LLVM bitcode files for instrumentation analysis. After cleaning the compilation commands (e.g., removing clang-incompatible flags), we recompile to produce x86-equivalent object files for each source.

\input{tables/gcc_clang_differences}

\input{listings/inlineASM}

\input{listings/hexASM}

\subsubsection{Human-In-Loop Approach to Resolve Compilation Errors:}
~\systemname{} monitors the compilation process and fixes any errors which are caused by known issues. Some of the common issues which framework resolves in a semi-automated way are - 

\subsubsection*{(1) GCC vs Clang Incompatibilities:}
\label{subsec:compiler_diffs}

A significant portion of open-source embedded software relies on GCC-based toolchains~\cite{von2011definitive}, making the transition from a GCC build environment to Clang challenging. Table~\ref{tab:gcc_clang_diffs} highlights several incompatibilities between GCC and Clang~\systemname{} that we identified during the process of porting. Although clang's official documentation does highlight some of the incompatibilities of Clang against GCC~\cite{LanguageCompatibility}, we believe we are the first to highlight these issues in the embedded domain, which have not yet received sufficient attention among embedded developers. Addressing these incompatibilities can help facilitate effective cross-compiler compatibility. Issues like Variable-Sized Object initialization are still not supported even in the latest version of LLVM at the time of writing (LLVM 18)~\cite{dgookin_2023}. The table also highlights challenges such as absence of certain symbols like \textit{\_\_assert\_func} which are internal to Arm GCC's intrinsic header files. For these symbols, we capture their corresponding definitions from the original source's preprocessor output. We create a global header file which is then included in the subsequent compilation. Most of the compiler error fixing is automated via pattern matching and patching source code with accurate fixes, examples of which are provided in Table~\ref{tab:gcc_clang_diffs}. However, for other issues which we could not automate,~\systemname{} provides hints to developers to assist in fixing them.

\subsubsection*{(2) Handling Inline Assembly:}
% \ritvik{Add challenges wrt how hard it is to identify inline asm on source level - say how clang AST parser fails to grab ASM from inside macros and source level parsing to extract such ASM is tedious task.}
Our observations indicate that most \ritvik{Quantify how much} inline assembly in embedded applications is used for board-specific startup and initialization. This step is generally not necessary for the application to function as intended on the Linux platform. \systemname{} identifies all such assembly snippets throughout the application's code base and nops them during compilation. Identifying inline assembly at the source level poses challenges, especially when it is embedded within macros. Tools like Clang’s AST parser often fail to extract inline assembly from such constructs, making source-level parsing complex and labor-intensive. Due to the complexity of inline assembly representation, \systemname{} may occasionally miss inline assembly in macro definitions. In such cases, developer assistance, guided by \systemname{}'s hints, may be needed to address the issue. The framework detects inline assembly based on pattern matching and other similar techniques, but there are other different ways in which application developers choose to depict inline assembly. Listing~\ref{lst:hexASM} shows a snippet from a function which uses hexadecimal code to represent inline assembly.~\systemname{} is capable of identifying this type of assembly based on how this hex code is used (as a function pointer in this example). We also observed that some applications use inline assembly functions to optimize reading values from architecture-specific registers, as shown in Listing~\ref{lst:inlineASM}. These values are often used in various program-specific initialization checks. Currently, we over-approximate these reads by returning 0 or 1 based on random numbers. While this approach can potentially lead to false positive crashes or unintended application behavior, we hypothesize that over multiple runs, this approximation will allow the application to overcome initialization routines where it might otherwise result in unexpected behaviour. 

\subsubsection*{(3) Identify ISRs and Integrate ISR Task:}
To ensure an embedded application runs correctly on a Linux platform, we insert an Interrupt Triggering Task. It operates alongside other tasks, periodically issuing interrupts to mimic real-time scenarios. If the application adheres to our requirements (See Section~\ref{subsec:app_requirements}), we identify all triggerable interrupt routines through the Interrupt Vector Table, typically located in board-specific startup files. \systemname{} filters interrupts based on whether calling the ISR directly from within the application's task would leave the application in an inconsistent state. This is determined by ensuring that the global structures responsible for handling the interrupt are properly initialized ~\ritvik{Include a listing showing uninitialized ISRs}. The task creation and scheduler checking APIs must be manually identified when porting applications to a new RTOS.

\subsubsection{Posix Swap}
After porting the application source files to x86, ensuring utilization of the Linux Portable Layer (LPL) in the underlying RTOS is crucial. This translates application-level semantics effectively into the POSIX environment. \systemname{} compiles a sample application separately for the POSIX board to utilize LPL. This process provides RTOS kernel files configured for the POSIX platform. We term this procedure as POSIX swap.

However, the original build instructions of the application may include board-specific configurations enabling certain HAL-specific APIs necessary for its function. Sometimes, peripheral models implemented in the original RTOS may not be available in the corresponding LPL, as discussed in Section~\ref{subsec:portability_layers}.

Addressing these challenges, \systemname{} selectively incorporates configurations from the application that do not disrupt the POSIX build. Each RTOS configuration is iteratively toggled in the POSIX build, saving configurations that compile successfully. Once the POSIX build incorporates necessary application configurations without issues, \systemname{} replaces the application's RTOS kernel files with those from the successful POSIX build.

\subsubsection{Resolve Linker Level Errors}

After the POSIX Swap, the final phase in porting an application is linking all object files. Replacing RTOS kernel object files with POSIX Kernel object files introduces two challenges~\ritvik{This approach can be explained algorithmically}:
\begin{itemize}
    \item \textbf{Undefined reference errors:} Occur when symbols referenced in the board-specific RTOS kernel files are absent in the POSIX Kernel files post POSIX swap.
    \item \textbf{Multiple reference errors:} Arise when symbols are duplicated across the swapped POSIX kernel files and the remaining application RTOS files.
\end{itemize}

\subsubsection*{(1) Resolving Undefined References}

To resolve undefined references, the framework looks for the corresponding application kernel object files which have this symbol defined. Bringing in this application kernel object file into linking can cause other multiple reference errors due to the symbols being defined in both application and the POSIX RTOS file. Some symbols like \emph{\_\_compiler\_barrier} are internal to the target architecture compiler for which we create dummy function signatures and empty bodies~\ritvik{Our Goal here is to maintain decent fidelity to enable security analysis on apps, so this is ok to do}. 

\subsubsection*{(2) Resolving Multiple References}
To resolve multiple references,~\systemname{} follows 2 phases. 

\begin{itemize}
    \item \textbf{Creating Library Archives :} By following the original build procedure of an application step by step, we observed that library archives are created by grouping certain object files together and are included during linking. This helps in linking object files of different modules where some object files in a module may have a symbol weakly defined whereas strongly defined in others. Archiving an object file with weakly defined symbol prevents occurrence of multiple reference errors ~\ritvik{Give an example of how RTOS apps use archiving.} .~\systemname{} identifies all the library archives that were created in the original build, thereby also capturing the information about which files have to be archived. This resolves large majority of multiple reference errors.

    \item \textbf{Modifying Symbol in One of the Objects:} The remaining multiple references cannot be resolved by archiving, hence the symbol name has to be modified in one of the object files. If the multiple reference is between an Application's object file~\ritvik{By App, we mean App + App kernel + App HAL} and POSIX kernel object file, we pick the Application object file for symbol modification; this is to ensure that we retain any calls that the application API makes into the POSIX layer of the RTOS. For other cases, we modify either of the object files to resolve the error.
\end{itemize}


\subsubsection{Handling RTOS Standard Library Calls}

Amidst our efforts in rehosting the application, we identified that, for an application to function as intended on a POSIX board, we must mimic the behavior introduced by the linker in symbol renaming when compiling a sample application for POSIX board. Mature RTOSes such as Nuttx and Zephyr employ sophisticated symbol management and linking strategies to handle the dual-context execution between the RTOS environment and the host system. This architecture creates a clear separation between the calls of RTOS standard library functions from the host through a specialized linking process. To mimic this behavior in our ported applications, we read the Global Offset Table (GOT) entries of the sample application to identify functions that should be directed to the host standard library. This allows us to determine which calls should be redirected to the application and which should be directed to the RTOS standard library.

\subsubsection{Handling Symbol Aliasing}
During testing of the ported application, we discovered that several null pointer dereference crashes were caused by attempts to call aliased symbols. In the original application's build procedure, the linker creates aliases for various symbols to maintain interoperability across different boards as guided by linker scripts. For instance, the symbol \textit{\_\_init\_clock} might be resolved to aliases like \textit{\_\_stm32\_clock\_init} or \textit{\_\_nrf52\_clock\_init}, depending on the target board. Additionally, multiple aliases can be created for the same symbol, further complicating our rehosting efforts. To address this, \systemname{} extracts aliasing information from the original ELF compiled for the board by loading the ELF in GDB and verifying which symbol each alias points to. With this information, our instrumentation passes ensure that all such aliases are correctly redirected to their original references at link time.




% \subsubsection*{(f) Handling Library Calls}

% \ritvik{Need to fill this now that it's done!}

% To preserve application fidelity on top of instrumentation, ~\systemname{} ensures that all calls to standard library are redirected to the application standard library (if one exists or is provided by the RTOS kernel). 

% \begin{itemize}
%     \item Capture Compilation Commands
%     \item Retarget for x86 ISA and handle inline assembly.
%     \item Resolve GCC vs Clang Issues.
%     \item Identify ISRs and Insert ISR Task.
%     \item Identify portable layer and replace with LPL.
%     \item Resolve Linker Level Errors.
%     \item Add stub methods for missing functions.
% \end{itemize}
\subsection{Handling Peripheral Interactions}

To handle peripheral interactions, \systemname{} performs the following 2 steps - 

\subsubsection{Constant Address Analysis}
Most MMIO address references in the ported application are constants. Our analysis identifies such constants in operands of load and store instructions, as well as constant arguments in function calls. We focus on addresses greater than 4 bytes and below the 32-bit userspace stack range to detect most MMIOs. Although some non-MMIO constants may also be flagged as MMIOs, providing input from stdin to these non-MMIO loads does not affect program behavior, as these constants are simply numbers and are not mapped to the ELF userspace in any way. Once we identify an MMIO address, we mask its value to the nearest page boundary. We then treat all MMIO accesses within a range of ±2 KB from that boundary as MMIOs. This approach helps group related MMIO accesses and ensures that accesses within the same memory-mapped region are consistently recognized.
% \begin{itemize}
%     \item Find constant addresses.
%     \item Coalescing adjacent Pages.
% \end{itemize}
\subsubsection{Memory Access Instrumentation}
We instrument all memory loads and stores so that the loads read from the standard input.

\subsection{Assisting Dynamic Analysis}

\PA{I think there should be a subsubsection here as this paragraph is about one effort to assist dynamic analysis. The subsection paragraph should provide an overview of the different efforts the subsection talks about}

As demonstrated by Liyanage et al.~\cite{reachableCoverage}, focusing on reachable coverage elements is key to enhancing fuzzing effectiveness by ensuring that only reachable code paths are tested. Building on this insight, we introduce a customized coverage metric for application-level fuzzing that focuses on all reachable functions from \textit{main} and \acp{ISR} injected by \systemname{} during the porting process. AFL++'s coverage, which reports the coverage of the entire program—including modules from the application’s kernel, the HAL, and the POSIX kernel—does not align well with our scenario. This broader coverage can be inaccurate, as it may include functions that are not reachable from the application's perspective. Our linking procedure brings in additional application kernel files to resolve undefined references, which may contain functions unused by the ported application.

\subsubsection{Reachability Analysis For Precise Coverage Measurement}

Our analysis traverses call graphs on the basic block level via LLVM IR and identifies all the functions reachable from \textit{main} and the ISRs that are injected by \systemname{}. However, when applications do not comply with our system requirements (see Section \ref{sec:threat_model}) and no ISRs are injected, we only get the reachable functions from main.

\subsubsection{Weakening data-independent conditions}

\input{listings/branch_instrument}

Our analysis found that certain conditions depend on MMIO values, creating constraints that AFL struggles to solve within a reasonable timeframe. Listing \ref{lst:blocker} illustrates one such constraint, which halts fuzzing thereby hindering our efforts in effective dynamic analysis of the application. While AFL++ could eventually resolve these constraints given enough time, they frequently appear early in board initialization routines, causing the application to remain stuck without progress. To address this, inspired by prior work \cite{choi2019grey}, we simplify MMIO-dependent constraints. Our instrumentation identifies such branches and modifies them to be controlled by \textit{stdin \% 2}, toggling the condition with a 50\% probability to give AFL a fair chance to explore both the if and else paths.

\section{Application Level Fuzzing}

We compile the instrumented bitcode with Sanitizers and use our modified AFL++ to fuzz the ported applications under persistent mode. Every MMIO access we have modeled will receive mutated inputs from AFL. Without any instrumentation, in configuration \textit{C0}, we observed that applications even failed to run RTOS related initialization tasks and result in no coverage. \textit{C1} configuration is coverage without any branch instrumentation or cross-function MMIO tracking, and \textit{}{C2} is coverage with data independent branches instrumented and cross-function MMIO tracking. Weakening of data independent conditions helps AFL cover more paths as can be seen in the coverage differences between both configurations of Lemix in Table~\ref{tab:tool_eval}. Our original coverage metric is source line coverage, which had to be normalized to basic block coverage to compare against existing works. \textit{C3} configuration is~\systemname{}'s application level coverage added to the unique number of basic blocks identified via function level fuzzing in functions that were not covered by application level fuzzing in \textit{C1}.

\section{Function Level Fuzzing}
Given a function, we will automatically create fuzzing harness.

\subsection{Type Inference and Co-Relation Analysis}

Type inference involves automatically identifying the types of inputs, outputs, and internal variables in a function.
This is crucial to ensure that the fuzzing harness understands the data structure and boundaries for each function. The fuzzing engine analyzes the function’s signature, its control flow, and the expected data types for each parameter.
Additionally, co-relation analysis is employed to understand how different variables or parameters within the function interact with each other.
This analysis allows the creation of relationships between the input variables and their potential effects on the function's behavior, ensuring that the generated test cases are meaningful and explore different paths within the function.

\subsection{Type Generation}

After type inference, type generation focuses on producing valid input values for the identified types.
This process involves mutating the inputs to cover a wide range of test cases, from edge cases to typical scenarios, while respecting the type constraints identified in the previous step.
For example, if a function accepts an integer, the type generation process will create a range of integers, including negative numbers, large values, and boundary cases.
If the function accepts a pointer or reference type, the type generation will include valid and invalid memory addresses.
The goal is to generate a comprehensive set of inputs that stress-test the function's handling of various types, ensuring that vulnerabilities or undefined behaviors are uncovered.

\subsection{Function Fuzzing}

Each target function is isolated into a standalone executable by accurately setting up its runtime environment, including arguments, global variables, and mocked dependencies, ensuring it is self-contained and behaves as expected.
A non-crashing seed input, identified automatically, is used as the input for AFL++, which further generates mutated inputs to explore various execution paths. Integrated sanitizers then detect and report any crashes or undefined behavior, enabling comprehensive vulnerability triaging.



==> sections/overview.tex <==
\section{Overview}
\label{sec:approach}
% \ritvik{Ready for review (needs work still)}
% \machiry{Briefly explain what is our approach--- i.e., rehost embedded application as linux applications. Such that all the necessary functionality is preserved and we can use existing techniques to test these applications.}

\systemname{} aims at providing a semi automated framework to help rehost embedded applications as x86 Linux executables to enable traditional security analysis of embedded software. Our framework currently works out of the box for major open source RTOSes including FreeRTOS, Zephyr, Nuttx, Threadx but with minimal configuration changes, it can easily be extended to other RTOses as well. Porting an application to Linux using \systemname{} comprises of  3 phases - first is the generation of x86 equivalent bitcode files from the RTOS Application source files. This includes the application source files as well as any device driver peripheral source files. The 2nd phase consists of compiling the supported RTOS with the x86 LLVM compiler using a demo application configured for the POSIX board to leverage the Linux Portable Layer. The RTOS kernel bitcode files are hence collected from this phase. The 3rd phase involves merging and integrating the RTOS core files compiled for x86 with the application and driver files from phase 2.


% \input{figures/lemix_design_phase1}

\subsection{Lemix Approach}
\label{subsec:overview}
\machiry{The goal here is to briefly explain how we solve our challenges.}
\machiry{Draw a figure }
To address challenges from Section~\ref{sec:challenges}, \systemname{} employs the following techniques -

\subsubsection*{(1) Rehosting as Dynamic Analysis Friendly Linux Application:}

The goal is to produce an x86-64 Linux binary hosting the given embedded application.,~\ie{} to produce a~\elx{} binary.
The generated binary also has instrumentations that improve the coverage and bug-detection capabilities of dynamic analysis techniques.

% \input{figures/lemix_design_phase2}

\subsubsection*{(2) Retargetting:}

Given a embedded application and the target~\ac{RTOS}, we use the linux portable layer of the~\ac{RTOS} and convert the embedded application into a x86-64 Linux application.
We use an interactive technique to handle the challenges in ISA re-targetting. This is done via minimal source level modifications to ISA specific application code. We also add a special dispatcher task that will mimic interrupts by invoking application interrupt handlers at regular intervals.

\subsubsection*{(3) Handling Peripheral Interactions:}

A constant address analysis is performed to find out~\ac{MMIO} ranges that can be accessed by the application.
We instrument loads and stores, such that, at runtime all loads from~\ac{MMIO} ranges will be converted into reads from standard input and all stores will be ignored.

\subsubsection*{(4) Instrumentation to Assist Dynamic Analysis:}

\iffalse
We use an enchanced ASAN instrumentation to handle custom memory management functions.
Using static analysis, we identify peripheral state constraints and add the necessary instrumentation to relax them.
\fi
To help fuzzers achieve better coverage in fuzzing, we perform instrumentation to ease data independent conditions if they are affected by~\ac{MMIO}. This is done in a way to minimize false positives that may arise due to constraint easing. We also evaluate our framework with and without the instrumentation to assess improvements in coverage and detection.

% \input{figures/lemix_design_phase3}

\subsubsection*{(5) Fuzzing}
The goal is to fuzz test the provided~\elx{} application.
We explore two testing modalities : (i) Application mode and (ii) Function mode.

In application mode, we test the whole application.  As mentioned in~\sect{sec:background}, embedded applications are continuously running applications and process inputs in each iteration.
We modified~\afl{}~\cite{fioraldi2020afl++} for this purpose.

In function mode, we directly fuzz test an arbitrary function in a given~\elx{} application.
However, as we explain in~\sect{sec:challenges}, there are various challenges in achieving this.
We use a combination of static analysis and type inference to solve these challenges. Finally, vulnerabilities will be reported with the appropriate crashing input and program trace.
%functions might have preconditions and invoking functions without satisfying these preconditions might result in false positive crashes.
%We use static analysis to solve these challenges and 





==> sections/overview2.tex <==
\section{Overview of Approach}

%Explain the overview of our approach using the overview figure.
Figure \ref{fig:overview} shows a high-level architecture of our rehosted application. As seen in the figure, the application tasks, third party SDK and RTOS are bundled together as a linux executable. In this section, we discuss the challenges involved in building, executing and handling inputs in the rehosted application and our approach towards solving them.

% Explain the two challenges and how to solve each of them:
\subsection{Building the Rehosted Application}

Embedded applications are designed to run on microcontrollers, which provides their own compiler toolchains and instruction sets. Running them on linux require compiling the source code with linux-based compilers, which reveal a number of challenges.

\textit{Challenges}
\begin{itemize} 
    \item \textbf{Inline assembly code: } To configure the hardware, embedded applications usually contain inlined assembly code which are specific to the instruction set of the MCU architecture. As a result, these application would not build and run if compiled with the linux toolchain.

    \item \textbf{Compiler-dependent semantics: } Embedded applications are also written following some language features and semantics specific to the MCU architecture such as dynamic variable declarations and pointer casts. Some of these features may not be supported by the linux architecture. 

     \item \textbf{Unsupported build arguments: } Embedded applications contain Makefiles that contain the hardware-specific toolchain, as well as build arguments, compiler and linker flags that may either not be supported by the linux compiler, or implemented with a different behavior. Example, the arm toolchain specifies the x flag which isn't supported by the x86 compilers and architecture. 
\end{itemize}

\textit{Our Approach}

Given these challenges, the first step to rehosting an embedded application is to set up a build file (Makefile) that is compatible with the linux environment. Our Makefile specifies the linux compiler and only its supported flags. We removed unsupported compiler flags because that are not required by the linux compiler. We also removed the the inlined assembly code because they were only used to setup the microcontrollers and peripherals. Finally, we rewrote the compiler-dependent codes in the application with language semantics that are compatible with the linux environment.


% 1. Preserving execution semantics: Explain the challenge (refer to intro).
% How do we handle this:
\subsection{Preserving execution semantics}

Embedded applications are designed following a task-based architecture. Whenever a higher priority task is waiting, the RTOS scheduler context-switches and schedules the higher priority task. In addition to these, functionalities in embedded applications are triggered by interrupts. To successfully rehost embedded applications, these semantics should be retained. Unfortunately, to rehost to a linux environment, this poses the following challenges:

\textit{Challenges}

\begin{itemize}
    \item \textbf{Thread-based context-switching: } The linux scheduler context-switches processes. Multiple threads are designed to run concurrently in a single process. Embedded applications consist of multiple tasks, with only one task running at a time. This difference in architecture prevents the preservation of the task-based execution in linux.
    
    \item \textbf{Interrupts are hardware-dependent: } Functionalities, and hence, code implementations, are triggered by interrupts. These interrupts are triggered by peripherals. By rehosting embedded applications to linux, we hope to remove the need for these peripherals, while still triggering the functionalities and preserving the application semantics. 
\end{itemize}

\textit{Our Approach}

To preserve the task-based semantics of embedded application, we substitute the MCU portable layer of the RTOS with the linux portable layer. The popular RTOSes already provide portable layer for the linux environment and hence, we only need to add the C files of the provided linux portable layer to the embedded application. To trigger functionalities that depend on interrupts, we designed an interrupt dispatcher as a separate high-priority task that calls the interrupt handlers dependent on by the application. To identify these handlers, we hook into the interrupt-registering routine and record the addresses of the interrupt handlers. These addresses are used by the interrupt dispatcher to invoke the various interrupt routines.

% 2. Handling peripherals: 
\subsection{Handling Peripheral Interactions}

Embedded applications interact with peripherals by reading from and writing into registers and memory location mapped to these peripherals. These peripherals influence application functionalities and hence, need to be handled. Unfortunately, this poses the following challenges:

% Briefly explain the challenge (Refer to the intro)
\textit{Challenges}

\begin{itemize}
    %Identifying peripheral accesses?
    \item \textbf{Identifying peripheral accesses:} Peripheral accesses are represented by either registers or hardcoded addresses in embedded applications. To properly handle these peripherals, we need to know which registers or memory addresses represent peripherals, different from normal application data.

    %How do we handle peripheral access?
    \item \textbf{Handling peripheral accesses:} Given the absence of peripherals, their accesses in the application need to be correctly handled. In addition to this, the peripheral addresses are usually encoded in the application and these address space would not belong to the application process in the linux environment, leading to illegitimate access.
\end{itemize}

\textit{Our approach}

From our review of embedded applications, we observed that peripheral addresses are defined in a MCU-dependent configuration file. Hence, to identify peripheral accesses in the application, we used the variable names defined in this file. % What about peripheral accesses represented as registers?
Handling peripheral accesses require both reading and writing to registers and addresses mapped to peripherals. Because  writing to peripherals do not directly change the application execution, we removed all writes to peripheral addresses. We replace all peripheral reads with reads from standard inputs. With dynamic analysis and coverage feedback, we can learn and feed in legitimate inputs that the application expects. Finally, we identify peripheral-based registers that are used in conditionals, but whose values are not used inside the conditional-block. We make these conditions to always be true so we can achieve maximum coverage. This approach was used by T-Fuzz~[CITE] and they demonstrated the effectiveness of ignoring such non-data dependent conditions for improving code coverage. 

%% I think this should be in the background
Listing~\ref{lst:isr} shows a snippet of an interrupt service routine that reads data from the USART1 peripheral. The status bits of \texttt{USART1} peripheral register are checked to determine if \texttt{USART1} has any data ready to be received. Upon meeting this condition, the received data is placed on the \ac{RTOS} queue, which other tasks can utilize thereby improving code coverage. Our analysis revealed that most of these conditions in place were non-data-dependent. By setting this condition to true, this block always executes. We also modified this code so that cChar is read from standard input and fed to the xUsart1\_RxQueue shown above. With advancements in dynamic analysis, we can get the actual values expected by the queue.  

%--GIVE AN EXAMPLE OF IF CONDITION--.

\input{listings/ifcond}

\subsection{Threat Model}
% --Provide clarification on threat model--i.e., we assume peripherals to be malicious.
Our design is based on the assumption that peripherals form the attack vectors for malicious actors. As for the non-critical peripherals, which are exposed to external agencies this assumption holds true. In the case of critical peripherals, we assume that it can be malformed and provide values which are not expected by the application code. 


==> sections/threat_model.tex <==
\section{Threat Model}
\label{sec:threat_model}

\input{figures/threat_model}

\ritvik{Make a stronger claim of why our threat model assumes MMIOs from attacker.}

In our threat model, illustrated in Figure~\ref{fig:threat_model}, we consider the security implications of an embedded application built on a Real-Time Operating System (RTOS), a type-2 embedded system. The primary focus is on malicious inputs originating from Memory Mapped Input/Output (MMIO) and interrupts, both of which are critical for how embedded systems interact with external stimuli.

\subsection{Application Specific Design Requirements}
\label{subsec:app_requirements}
During the process of porting an application, \systemname gathers information about all triggerable interrupts from the Interrupt Service Routine (ISR) vector table, which is typically found in board-specific startup files, often written in the native architecture's assembly language. \systemname identifies these startup files by analyzing the original application's compilation database. However, if the application defines and uses custom ISRs, these startup files might not include the ISR vector table. Consequently, if such a file is not located, ISRs may not be simulated as intended by our design.

\input{listings/fuzz_ability}

We assume that the embedded application operates within a constrained environment, typical of RTOS-based systems, where resources such as memory and processing power are limited. The system is expected to interact with hardware peripherals through MMIO, and it relies on interrupts for timely response to external events. Listing~\ref{lst:fuzz_ability} depicts how MMIOs get instrumented and behave according to our threat model.

\subsection{Adverseries}

Attackers with physical or remote access to the device who can control or craft malicious inputs to MMIOs or trigger interrupts in a way that can create a possibility of memory exploits~\cite{arroyo2021a}. A malicious peripheral may therefore not abide by the agreement with the device specifications and send malicious data to the application, resulting in undefined behavior, denial of service, or worse case, resulting in arbitrary code execution \cite{ma2022printfuzz}. Additionally, in the case of essential peripherals (\eg clock), any deviation from the valid behavior could possibly create a scenario that is not expected (\eg disabling a safety mechanism)~\cite{CANNON}


==> tables/dataset_table.tex <==
\begin{table}
\tiny
\caption{Summary of our Dataset containing 18 applications across four prevalent RTOSes.
The SLOC (Source Lines of Code) column counts code from the application source files, headers, assembly files, SDKs and submodules used by the application, and the underlying RTOS.
(\tbl{tab:full_dataset_table} in Appendix has full details).}
\vspace{0.25cm}
\scriptsize
\centering
\renewcommand{\arraystretch}{1.5}
\begin{tabular}{clcr}
\toprule
\textbf{RTOS} & \textbf{Application} & \textbf{ID} & \textbf{SLOC} \\ 
\midrule
\multirow{5}{*}{FreeRTOS} 
& \cellcolor[HTML]{EFEFEF}FlipperZero & \cellcolor[HTML]{EFEFEF}f1 & \cellcolor[HTML]{EFEFEF}289k \\
& Infinitime & f2 & 2.39M \\
& \cellcolor[HTML]{EFEFEF}SmartSpeaker & \cellcolor[HTML]{EFEFEF}f3 & \cellcolor[HTML]{EFEFEF}172.8k \\
& cdc\_msc\_freertos & f4 & 933k \\
& \cellcolor[HTML]{EFEFEF}hid composite freertos & \cellcolor[HTML]{EFEFEF}f5 & \cellcolor[HTML]{EFEFEF}932k \\ 
\midrule
\multirow{5}{*}{Nuttx}
& nrf52840-dk pwm & n1 & 2.1M \\
& \cellcolor[HTML]{EFEFEF}nrf52-feather i2c & \cellcolor[HTML]{EFEFEF}n2 & \cellcolor[HTML]{EFEFEF}2.02M \\
& nsh & n3 & 2.07M \\
& \cellcolor[HTML]{EFEFEF}spawn & \cellcolor[HTML]{EFEFEF}n4 & \cellcolor[HTML]{EFEFEF}2.1M \\
& PX4-Autopilot & n5 & 1.9M \\ 
\midrule
\multirow{3}{*}{Zephyr}
& Zephyr Blinky & z1 & 20.2k \\
& \cellcolor[HTML]{EFEFEF}zmk & \cellcolor[HTML]{EFEFEF}z2 & \cellcolor[HTML]{EFEFEF}28.6k \\
& ZSWatch & z3 & 36.6k \\ 
\midrule
\multirow{5}{*}{Threadx} 
& Tx\_FreeRTOS\_Wrapper & t1 & 1.09M \\
& \cellcolor[HTML]{EFEFEF}Tx\_LowPower & \cellcolor[HTML]{EFEFEF}t2 & \cellcolor[HTML]{EFEFEF}922k \\
& Tx\_Module & t3 & 1.01M \\
& \cellcolor[HTML]{EFEFEF}Tx\_Thread\_Creation & \cellcolor[HTML]{EFEFEF}t4 & \cellcolor[HTML]{EFEFEF}871k \\
& Tx\_Thread\_MsgQueue & t5 & 996k \\
\bottomrule
\end{tabular}
\label{tab:dataset_table}
\end{table}

==> tables/implementationtable.tex <==
\begin{table}[]
\caption{Implementation summary of \systemname{} components. \machiry{Ritvik, fix this.}}
\vspace{0.25cm}
\begin{tabular}{c|c|c|c}
\toprule
\textbf{Phase}     & \textbf{Component}                                                       & \textbf{language} & \textbf{SLoC} \\ 
\midrule
\multirow{4}{*}{1} & \elapp{} generation                                                         & Python, C++            &       6.5k, 1.06k        \\ \cline{2-4} 
                   & MMIO handling                                                            & C++               &        1.1k       \\ \cline{2-4} 
                   & \begin{tabular}[c]{@{}c@{}}Dynamic \\ Analysis\\ Assistence\end{tabular} & C++               &        983       \\ \cline{2-4} 
                   & \begin{tabular}[c]{@{}c@{}}Runtime\\ Library\end{tabular}                & C                 &        383       \\ \hline
\multirow{2}{*}{2} & \begin{tabular}[c]{@{}c@{}}AFL++ \\ Modifications\end{tabular}           & C                 &        100       \\ \cline{2-4} 
                   & \begin{tabular}[c]{@{}c@{}}Function Level\\ Fuzzing\end{tabular}         & C/C++             &               \\ \bottomrule
\end{tabular}
\label{tab:imlementationable}
\end{table}
